Counting and enumerating optimum cut sets for hypergraph $k$-partitioning problems for fixed $k$

We consider the problem of enumerating optimal solutions for two hypergraph $k$-partitioning problems -- namely, Hypergraph-$k$-Cut and Minmax-Hypergraph-$k$-Partition. The input in hypergraph $k$-partitioning problems is a hypergraph $G=(V, E)$ with positive hyperedge costs along with a fixed positive integer $k$. The goal is to find a partition of $V$ into $k$ non-empty parts $(V_1, V_2, \ldots, V_k)$ -- known as a $k$-partition -- so as to minimize an objective of interest. 1. If the objective of interest is the maximum cut value of the parts, then the problem is known as Minmax-Hypergraph-$k$-Partition. A subset of hyperedges is a minmax-$k$-cut-set if it is the subset of hyperedges crossing an optimum $k$-partition for Minmax-Hypergraph-$k$-Partition. 2. If the objective of interest is the total cost of hyperedges crossing the $k$-partition, then the problem is known as Hypergraph-$k$-Cut. A subset of hyperedges is a min-$k$-cut-set if it is the subset of hyperedges crossing an optimum $k$-partition for Hypergraph-$k$-Cut. We give the first polynomial bound on the number of minmax-$k$-cut-sets and a polynomial-time algorithm to enumerate all of them in hypergraphs for every fixed $k$. Our technique is strong enough to also enable an $n^{O(k)}p$-time deterministic algorithm to enumerate all min-$k$-cut-sets in hypergraphs, thus improving on the previously known $n^{O(k^2)}p$-time deterministic algorithm, where $n$ is the number of vertices and $p$ is the size of the hypergraph. The correctness analysis of our enumeration approach relies on a structural result that is a strong and unifying generalization of known structural results for Hypergraph-$k$-Cut and Minmax-Hypergraph-$k$-Partition. We believe that our structural result is likely to be of independent interest in the theory of hypergraphs (and graphs).

==> enumeration-algorithm-simple.tex <==
\section{Enumeration Algorithm} \label{sec:enumeration-algorithm}

We will use Theorems \ref{theorem: structure thm 1} and \ref{theorem: structure thm 2} to design a deterministic polynomial-time algorithm for \enumhkcut in this section. 
%For a hypergraph $G=(V,E)$ and vertex set $U\subseteq V$, we recall that $G[\complement{U}]$ denotes the subhypergraph obtained by discarding $U$ and by discarding all hyperedges $e\in E$ with  $e\cap U\neq \emptyset$. 
%We will use $T(n,p)$ to denote the run time of a source minimal minimum $(S,T)$-terminal cut computation in an $n$-vertex hypergraph of size $p$. 
We describe the formal algorithm in Figure \ref{Algo: enum-cuts}. It enumerates $n^{O(k)}$ source minimal minimum $(S,T)$-terminal cuts and considers the cut-set crossing each cut in this collection. If the removal of the cut-set leads to at least $k$ connected components, then it adds such a cut-set to the candidate family $\family$; otherwise, it adds the source set of the cut into a candidate collection $\collection$. 
%For a minimum $k$-partition $(V_1, \ldots, V_k)$, by the structural theorems, either the collection $\collection$ is guaranteed to contain all parts $V_1, \ldots, V_k$ or the family $\family$ is guaranteed to contain $\delta(V_1, \ldots, V_k)$. 
Next, the algorithm considers 
%We account for the former possibility by considering 
all possible $k$-partitions that can be formed using the sets in the collection $\collection$ and adds the set of hyperedges crossing the $k$-partition to the family $\family$. Finally, it prunes the family $\family$ to return all minimum $k$-cut-sets in it. 
%This family is guaranteed to contain the cut-set of one of the parts of every minimum $k$-partition. The algorithm then recursively finds all minimum $(k-1)$-cuts-sets after removing the found cut-set and the associated source side. 
The run-time guarantee and the cardinality of the family of $k$-cut-sets returned by the algorithm are given in Theorem \ref{theorem: enum algorithm}. Theorem \ref{thm:enumhkcut-algo} follows from Theorem \ref{theorem: enum algorithm} by observing that the source minimal minimum $(S,T)$-terminal cut in a hypergraph can be computed in deterministic polynomial time---e.g., it can be computed in a $n$-vertex hypergraph of size $p$ in $O(np)$ time \cite{ChekuriX18}.  

% \begin{comment}
% \begin{algorithm}
% \caption{Enum-Cuts$(G=(V,E),k)$}
% \label{Algo: enum-cuts}
% \begin{algorithmic}[1]
% \IF{$k=1$}
% \STATE Return $\{\emptyset\}$
% \ELSIF{$k>|V|$}
% \STATE Return $\emptyset$
% \ELSE
% \STATE Initialize $\mathcal{C}\gets\emptyset$, $\mathcal{F}\gets\emptyset$
% \FOR{each pair $(S,T)$ such that $S,T\subseteq V$, $|S|,|T|\leq 2k-1$ and $S\cap T=\emptyset$}
% \STATE Compute the source-minimal minimum $(S,T)$-terminal cut $(U,\complement{U})$
% \STATE $\mathcal{C}\gets\mathcal{C}\cup\{U\}$
% \ENDFOR
% \FOR{each $U\in\mathcal{C}$}
% \STATE $\mathcal{F}_U\gets$Enum-Cuts$(G[\complement{U}],k-1)$
% \STATE $\mathcal{F}\gets\mathcal{F}\cup\{\delta(U)\cup F:F\in\mathcal{F}_U\}$
% \ENDFOR
% \STATE Return $\mathcal{F}$
% \ENDIF
% \end{algorithmic}
% \end{algorithm}
% \end{comment}

\begin{figure*}[ht]
\centering\small
\begin{algorithm}
\textul{Algorithm Enum-Cuts$(G=(V,E),k)$}\+
\\{\bf Input:} Hypergraph $G=(V,E)$ and an integer $k\geq 2$
\\{\bf Output:} Family of all minimum $k$-cut-sets in $G$
%\\ If $k=1$ \+
%\\ Return $\{\emptyset\}$\-
%\\ Else\+
\\ Initialize $\mathcal{C}\gets\emptyset$, $\mathcal{F}\gets\emptyset$
\\ For each pair $(S,T)$ such that $S,T\subseteq V$ with $S\cap T=\emptyset$ and $|S|,|T|\leq 2k-1$ \+
\\ Compute the source minimal minimum $(S,T)$-terminal cut $(U,\complement{U})$
\\ If $G-\delta(U)$ has at least $k$ connected components \+
\\ $\family\leftarrow \family\cup \set{\delta(U)}$\-
\\ Else \+
\\ $\mathcal{C}\gets\mathcal{C}\cup\{U\}$\-\-
\\ For each $k$-partition $(U_1, \ldots, U_k)$ of $V$ with $U_1, \ldots, U_k\in \mathcal{C}$ \+
\\ $\mathcal{F}\gets\mathcal{F}\cup\{\delta(U_1, \ldots, U_k)\}$\-
\\ Among all $k$-cut-sets in the family $\mathcal{F}$, return the subfamily of cheapest ones
\end{algorithm}
\caption{Algorithm to enumerate hypergraph minimum $k$-cut-sets}
\label{Algo: enum-cuts}
\end{figure*}
%\cnote{There shouldn't be a hyphen in "source minimal" in the third line of the algorithm.}

% \knote{Avoid periods in the above algorithm. You might want to use the same environment as in the file `basic-recursive-algorithm.tex'. }

%\knote{Use the environment as in the file `basic-recursive-algorithm.tex'. It boxes the algorithm nicely.}

% \knote{State the phrasing of the second structural theorem that you need to argue correctness in this section. Put it in that section.} 

\begin{theorem} \label{theorem: enum algorithm}
Let $G=(V,E)$ be a $n$-vertex hypergraph of size $p$ and let $k$ be an integer. Then, Algorithm Enum-Cuts$(G,k)$ in Figure \ref{Algo: enum-cuts} returns the family of all minimum $k$-cut-sets in $G$ and it can be implemented to run in $O(n^{4k-2})T(n,p)+O(n^{4k^2-2k}p)$ time, where $T(n,p)$ denotes the time complexity for computing the source minimal minimum $(s,t)$-terminal cut in a $n$-vertex hypergraph of size $p$. Moreover, the cardinality of the family returned by the algorithm is $O(n^{2k(2k-1)})$.
\end{theorem}


% \wnote{If the algorithm returns only min $k$-cut-sets in $\mathcal{F}$ instead of just $\mathcal{F}$, then the run time might be $n^{O(k^3)}$, because the last line needs $O(n^{2k^2}p)$ time in each recursion. If we return just $\mathcal{F}$, and check validity only at the very end, then the run time is still $O(n^{2k^2}T(n,p))$.}
% \knote{Shouldn't time to prune in the last line be the same as time to write the output. Each recursive call is anyway going to spend the time to write the output, so it might as well check it while writing the output? This seems to be an issue of how best to explain it.}

\begin{proof}
%\knote{use family for $\mathcal{F}$ and collection for $\mathcal{C}$ consistently in this section.}
We begin by showing correctness. 
The last step of the algorithm considers only $k$-cut-sets in the family $\family$, 
%All candidates considered by the algorithm Enum-Cuts$(G,k)$ correspond to $k$-cut-sets, 
so the algorithm returns a subfamily of $k$-cut-sets. We only have to show that every minimum $k$-cut-set is in the family $\family$; 
%returned by the algorithm; 
this will also guarantee that every $k$-cut-set in the returned subfamily is indeed a minimum $k$-cut-set. %We show this by induction on $k$.

%For the base case of $k=1$, the only minimum $k$-cut-set is the empty set which is contained in the returned family. We now show the induction step. Assume that $k\ge 2$. By induction hypothesis, the algorithm will return the family of all minimum $(k-1)$-cut-sets for every input hypergraph $G'$. 
Let $F\subseteq E$ be a minimum $k$-cut-set in $G$ and let $(V_1,\ldots,V_k)$ be a minimum $k$-partition such that $F=\delta(V_1,\ldots,V_k)$. We will show that $F$ is in the family 
$\mathcal{F}$. 
%returned by the algorithm.
We know that $d(V_i)\le \opt$ for every $i\in [k]$. We distinguish two cases:
\begin{enumerate}
    \item Suppose $d(V_i)<\opt$ for every $i\in [k]$.
    
    Consider an arbitrary part $V_i$ where $i\in [k]$. By Theorem \ref{theorem: structure thm 1}, there exist disjoint subsets $S,T\subseteq V$ with $|S|,|T|\leq 2k-2$ such that $(V_i,\complement{V_i})$ is the unique minimum $(S,T)$-terminal cut. Hence, the set $V_i$ is in the collection $\mathcal{C}$. 
    Consequently, all parts $V_1, \ldots, V_k$ are in the collection $\collection$. Hence, the set $F=\delta(V_1, \ldots, V_k)$ is added to the family $\family$ in the second for-loop. 
    
    %Moreover, $\complement{V_i}$ contains $k-1$ non-empty sets $V_2,V_3,\ldots,V_k$, so we have $|\complement{V_1}|\geq k-1$. Since $(V_1,\ldots,V_k)$ is a minimum $k$-partition, the set $F\backslash \delta(V_1)$ is a minimum $(k-1)$-cut-set in $G[\complement{V_1}]$. By induction hypothesis, we know that $F\backslash \delta(V_1)$ is contained in the family $\mathcal{F}_{V_1}$. Therefore, the set $F$ is contained in the family $\mathcal{F}$.
    
    \item Suppose there exists $i\in [k]$ such that $d(V_i)=\opt$.
    
    In this case, we have $\delta(V_i)=F=\delta(V_1,\ldots,V_k)$. By Theorem \ref{theorem: structure thm 2}, there exist disjoint subsets $S,T\subseteq V$ with $|S|,|T|\leq 2k-1$ such that the source minimal minimum $(S,T)$-terminal cut $(A,\complement{A})$ satisfies $\delta(A)=\delta(V_i)=F$. 
    Therefore, the set $F$ is added to the family $\family$ in the first for-loop. 
    %Therefore, the set $A$ is in the collection $\collection$. Since $A\subseteq V_1$ and $F=\delta(A)$, the hypergraph $G[\complement{A}]$ contains at least $k-1$ connected components. Hence, $|\complement{A}|\geq k-1$ and $F\setminus \delta(A)=\emptyset$ is a minimum $(k-1)$-cut-set in $G[\complement{A}]$. By induction hypothesis, we know that the empty set is contained in the family $\mathcal{F}_A$. Therefore, the set $F$ is contained in the family $\mathcal{F}$.
\end{enumerate}
Thus, in both cases, we have shown that the set $F$ is contained in the family $\mathcal{F}$. Since the algorithm returns the subfamily of hyperedge sets in $\mathcal{F}$ that correspond to minimum $k$-cut-sets, the set $F$ is in the family returned by the algorithm.

%\knote{Why should we care about $k>|V|$ in the algorithm separately? Explain it in the correctness proof. Perhaps along with the base case or after the proof of the induction step. I think a cleaner-fix to avoid this $k>|V|$ case is to have an additional condition: `For each $U\in \mathcal{C}$ with $|\complement{U}|\ge k-1$. Now add a proof in both cases that $|\complement{V_1}|\ge k-1$ and $|\complement{A}|\ge k-1$.}

% It remains to bound the cardinality of $\mathcal{F}$ and run time of Algorithm \ref{Algo: enum-cuts}. Let $N(k,n)$ denote the number of source-minimal minimum $(S,T)$-terminal cut computations in Enum-Cuts$(G,k)$ for an $n$-vertex hypergraph $G$. Then we have $N(1,n)=O(1)$. For $k\geq 2$, there are a total of $O(n^{4k})$ pairs $(S,T)$ such that $S,T\subseteq V$, $|S|,|T|\leq 2k-1$ and $S\cap T=\emptyset$. Hence, line 7-10 incurs $O(n^{4k})$ source-minimal minimum $(S,T)$-terminal cut computations, and the family $\mathcal{C}$ has $O(n^{4k})$ elements at line 10. For each $U\in\mathcal{C}$, the computation of Enum-Cuts$(G[\complement{U}],k-1)$ in line 12 incurs $N(k-1,n)$ source-minimal minimum $(S,T)$-terminal cut computations. Hence, line 11-14 incurs $O(n^{2k})N(k-1,n)$ source-minimal minimum $(S,T)$-terminal cut computations. Therefore, we have
% \[N(k,n)=O(n^{4k})+O(n^{4k})N(k-1,n),\]
% which implies $N(k,n)=O(n^{2k^2})$. Each hyperedge set in the output $\mathcal{F}$ requires at least one source-minimal minimum $(S,T)$-terminal cut computation \knote{This is not very clear. You might want to again bound this by induction on $k$? }, so we must have
% \[|\mathcal{F}|=O(n^{2k^2}).\]
% It also follows that the total run time of Algorithm \ref{Algo: enum-cuts} is $O(n^{2k^2}T(n,p))$.

%It remains to bound the cardinality of the family returned by the algorithm 
%$\mathcal{F}$ 
%and the run-time of Algorithm \ref{Algo: enum-cuts}.
Next, we bound the run time and the number of minimum $k$-cut-sets returned by the algorithm. The first for-loop can be implemented using $O(n^{4k-2})$ source minimal minimum $(s,t)$-terminal cut computations. Moreover, the size of the collection $\collection$ is $O(n^{4k-2})$. The number of tuples $(U_1, \dots, U_k) \in \mathcal{C}^k$ is $O(n^{4k^2-2k})$. Verifying if a tuple $(U_1, \dots, U_k)$ forms a $k$-partition takes $O(n)$ time. For a tuple which forms a $k$-partition, computing the hyperedges crossing that partition takes $O(p)$ time. Thus, the second for-loop can be implemented to run in time $O(n^{4k^2-2k}p)$. %$\binom{|\collection|}{k}=O(n^{2k(2k-1)})$ \cnote{This is the number of k-tuples that we need to consider, but it's not clear how to check whether a given tuple is a k-partition in constant time.}. 
The size of the family $\family$ is $O(n^{4k^2-2k})$. Each $k$-cut-set in $\family$ has representation size at most $p$. Hence, computing the size of each $k$-cut-set in $\family$ and returning the cheapest ones can be implemented to run in time $O(n^{4k^2-2k}p)$.
%Hence, the last step can be implemented to run in time $O(n^{2k(2k-1)})$.  
%(by doing two passes over the $\family$ and counting the number of hyperedges that cross). 
Thus, the overall run-time is $O(n^{4k-2})T(n,p)+O(n^{4k^2-2k}p)$.  
%\cnote{Should we use this bound in the theorem statement instead of $O(n^{4k})T(n,p)+O(n^{2k(2k-1)})?$}. 
%\wnote{Do we need to explain how to check optimality in constant time?} %\knote{It can be done in two passes over $\family$. Doesn't need explanation.}

%\knote{Verifying if a tuple $(U_1, \ldots, U_k)$ forms a $k$-partition takes $O(n)$ time. Each set in the family $\family$ has $O(m)$ hyperedges and each hyperedge has size $O(n)$ (Each set in the family $\family$ can be computed in $O(p)$ time). So, the run-time for the second for-loop should be $O(n^{2k(2k-1)+1}p)$?}

\end{proof}





==> mmh-algorithm-1.tex <==
\section{Algorithm for \enumMMh}\label{sec:enummmh-algo}
%For disjoint subsets $U_1, \ldots, U_k\subseteq V$, we define the $k$-tuple $(U_1, ..., U_k)$ to be a \emph{$k$-cut-set representative} if there exists a $k$-partition $(V_1, \ldots, V_k)$ such that $U_i\subseteq V_i$ and $\delta(U_i)=\delta(V_i)$ for all $i\in [k]$. 
%\minmax $k$-partition $(V_1, \ldots, V_k)$ if 

We recall that for a $k$-partition $(V_1, \ldots, V_k)$ and disjoint subsets $U_1, \ldots, U_k\subseteq V$, the $k$-tuple $(U_1, \ldots, U_k)$ is defined to be a \emph{$k$-cut-set representative} of $(V_1, \ldots, V_k)$ if $U_i\subseteq V_i$ and $\delta(U_i)=\delta(V_i)$ for all $i\in [k]$. 
%For disjoint subsets $U_1, \ldots, U_k\subseteq V$, we define the $k$-tuple $(U_1, \ldots, U_k)$ to be a \emph{$k$-cut-set representative} if there exists a $k$-partition $(V_1, \ldots, V_k)$ of the vertex set $V$ such that $U_i\subseteq V_i$ and $\delta(U_i)=\delta(V_i)$ for all $i\in [k]$. 
%We call a $k$-cut-set representative to be a \minmaxkcutsetrep if it is the cut-set representative of some optimum $k$-partition for \mmh. 
We first show that there exists a polynomial-time algorithm to verify whether a given $k$-tuple $(U_1, \ldots, U_k)$ is a $k$-cut-set representative. 

%Our first algorithm below shows that the problem of verifying if a given $k$-tuple of disjoint subsets $(U_1, \ldots, U_k)$ is a cut-set representative. 

\begin{theorem}\label{Thm: hyp minmax-1}
Let $G=(V,E)$ be a $n$-vertex hypergraph with $m$ hyperedges and let $k$ be an integer. 
%Let $(P_1, \ldots, P_k)$ be a $k$-partition and let $U_1, \ldots, U_k$ be arbitrary sets satisfying $U_i\subseteq P_i$ and $\delta(U_i)=\delta(P_i)$ for all $i\in [k]$. 
Then, there exists an algorithm that takes as input the hypergraph $G$ and disjoint subsets $U_1, \ldots, U_k$ and runs in time $O(nmk)$ to decide if there exists a $k$-partition $(V_1, \ldots, V_k)$ satisfying $U_i\subseteq V_i$ and $\delta(V_i)=\delta(U_i)$ for all $i\in [k]$ 
%(and hence, $\cup_{i=1}^k\delta(V_i)=\cup_{i=1}^k\delta(U_i)$), 
and return one if it exists. 
\end{theorem}
%\wnote{I dropped \minmax in this theorem because they don't have to be \minmax partitions to be recovered}

\begin{proof}
We will use Algorithm Recover-Partition$(G, U_1, \ldots, U_k)$ in Figure \ref{Algo: hyp minmax-1}. 


\begin{figure*}[ht]
\centering\small
\begin{algorithm}
\textul{Algorithm Recover-Partition$(G=(V,E),U_1,\ldots,U_k)$}\+
\\{\bf Input:} Hypergraph $G=(V,E)$ and disjoint subsets $U_1, \ldots, U_k\subseteq V$
\\{\bf Output:} Decide if there exists a $k$-partition $(V_1,\ldots,V_k)$ of $V$ with $U_i\subseteq V_i$ and $\delta(V_i)=\delta(U_i)$ $\forall i\in[k]$, \+\+
\\$\,\;$and return one if it exists\-\-
\\For each $i\in [k]$ initialize $P_i$ to be the union of the components of $G-\cup_{r=1}^k\delta(U_r)$ that intersect $U_i$ 
\\Let $C_1,\ldots,C_t\subseteq V$ be the components of $G-\cup_{i=1}^k\delta(U_i)$ that are disjoint from $\cup_{i=1}^k U_i$
%V_i\gets U_i$ $\forall i\in[k]$
\\For $j=1,\ldots,t$\+
\\If $\exists i\in [k]$ such that $\delta(P_i\cup C_j)=\delta(P_i)$\+
%\\For $i=1,\ldots,k$\+
%\\If $\delta(V_i\cup C_j)=\delta(V_i)$\+
\\$P_i\gets P_i\cup C_j$\-\- %and break\-\-
\\If $(P_1,\ldots,P_k)$ is a $k$-partition of $V$\+
\\Return $(P_1,\ldots,P_k)$\-
\\Else\+
\\Return NO
\end{algorithm}
\caption{Algorithm in Theorem \ref{Thm: hyp minmax-1}}
\label{Algo: hyp minmax-1}
\end{figure*}

We begin by showing correctness. 
%works as described in Theorem \ref{Thm: hyp minmax-1}.
Since Algorithm \ref{Algo: hyp minmax-1} maintains $U_i\subseteq P_i$ and $\delta(P_i)=\delta(P_i)$ for all $i\in[k]$, if it returns a $k$-partition, then the $k$-partition necessarily satisfies the required conditions. Next, we show that if a $k$-partition $(V_1, \ldots, V_k)$ satisfying the required conditions exists, then the algorithm will indeed return a $k$-partition $(P_1, \ldots, P_k)$ satisfying the required conditions (however, $(P_1,\ldots, P_k)$ may not necessarily be the same as $(V_1, \ldots, V_k)$). 

Let $(V_1, \ldots, V_k)$ be a $k$-partition such that $U_i\subseteq V_i$ and $\delta(U_i)=\delta(V_i)$ for all $i\in [k]$. Let $(P_1, \ldots, P_k)$ be the sequence of subsets at the end of the for-loop. Moreover, for each $j\in[t]$, let $(P^j_1, \ldots, P^j_k)$ be the sequence of subsets at the end of the $j$th iteration of the for-loop. For notational convenience, for $i\in [k]$, we will define $P_i^0$ to be the union of components of $G-\cup_{r=1}^k \delta(U_r)$ that intersect $U_i$ \cnote{Isn't "the union of components of $G-\cup_{r=1}^k \delta(U_r)$ that intersect $U_i$" just $U_i$? A component that intersects $U_i$ but contains a vertex outside of $U_i$ would have to have an edge in $\delta(U_i)$. }. We note that $(P_1, \ldots, P_k)=(P^t_1, \ldots, P^t_k)$ and that $P_i^0\subseteq P_i^1\subseteq\ldots\subseteq P_i^t$ for every $i\in[k]$. 
We observe that $U_i\subseteq P_i^j$ and $\delta(U_i)=\delta(P_i^j)$ for all $j\in \{0, 1, 2, \ldots, t\}$. Moreover, the subsets $P_1^j, \ldots, P_k^j$ are pairwise disjoint for each $j\in \{0, 1,2, \ldots, t\}$. Therefore, it suffices to show that $\cup_{i=1}^k P_i = V$. 

We claim that $C_1\cup\ldots\cup C_{j}\subseteq\cup_{i=1}^k P_i^{j}$ for each $j\in\{0,1,\ldots,t\}$. Applying this claim for $j=t$ gives that $\cup_{i=1}^k P_i=V$ as desired. We now show the claim by induction on $j$. The base case of $j=0$ holds by definition. 
We now prove the induction step. By induction hypothesis, we have that  $C_1\cup\ldots\cup C_{j-1}\subseteq\cup_{i=1}^k P_i^{j-1}$. 
We will show that there exists $i\in [k]$ such that $\delta(P_i^{j-1}\cup C_j)=\delta(P_i^{j-1})$. 
%$C_j\subseteq V_i^j$, i.e., $C_j$ is merged with one of the sets in $\{V_1^{j-1},\ldots,V_k^{j-1}\}$ by the inner for-loop. 
%To show $C_1\cup\ldots\cup C_{j}\subseteq\cup_{i=1}^kV_i^{j}$, we will show that $C_j$ is merged with one of $V_1^{j-1},\ldots,V_k^{j-1}$ in the inner for-loop. 
We know that $C_j$ is contained in one of the sets in $\{V_1, \ldots, V_k\}$, say $C_j\subseteq V_\ell$ for some $\ell\in [k]$. 
We will prove that $\delta(P_{\ell}^{j-1}\cup C_j)=\delta(P_{\ell}^j)$ to complete the proof of the claim. 
%We will prove that the inner for-loop can merge $C_j$ with $V_\ell^{j-1}$ by showing that $\delta(V_{\ell}^{j-1}\cup C_j)=\delta(V_{\ell}^{j-1})$. 
Since $C_j$ is a component of $G-\cup_{i=1}^k\delta(U_i)=G-\cup_{i=1}^k\delta(V_i)$, we know that each hyperedge in $\delta(C_j)$ crosses the $k$-partition $(V_1, \ldots, V_k)$. Moreover, each hyperedge in $\delta(C_j)$ intersects $C_j\subseteq V_\ell$, and hence,  $\delta(C_j)\subseteq \delta(V_\ell)$. Therefore,
\[
\delta(P_\ell^{j-1}\cup C_j)-\delta(P_\ell^{j-1})\subseteq \delta(C_j)\subseteq \delta(V_\ell)=\delta(U_\ell)=\delta(P_\ell^{j-1}).
\]
This is possible only if $\delta(P_\ell^{j-1}\cup C_j)-\delta(P_\ell^{j-1})=\emptyset$, i.e., $\delta(P_\ell^{j-1}\cup C_j)\subseteq\delta(P_\ell^{j-1})$. We now show show the reverse inclusion. We have that
\begin{align*}
    \delta(P_\ell^{j-1})-\delta(P_\ell^{j-1}\cup C_j)&=\delta(U_\ell)-\delta(P_\ell^{j-1}\cup C_j)
    \\&=\delta(V_\ell)-\delta(P_\ell^{j-1}\cup C_j)
    \\&=E(V_\ell-P_\ell^{j-1}-C_j,V-V_\ell-P_\ell^{j-1})\cup E(V_\ell\cap P_\ell^{j-1},P_\ell^{j-1}-V_\ell)
    \\&\subseteq E[V-P_\ell^{j-1}]\cup E[P_\ell^{j-1}].
\end{align*}
We note that the LHS is a subset of $\delta(P_\ell^{j-1})$ while the RHS is disjoint from $\delta(P_\ell^{j-1})$ since $E[V-P_\ell^{j-1}]\cap \delta(P_\ell^{j-1})=\emptyset$ and $E[P_\ell^{j-1}]\cap \delta(P_\ell^{j-1})=\emptyset$. Hence, the above containment is possible only if $\delta(P_\ell^{j-1})-\delta(P_\ell^{j-1}\cup C_j)=\emptyset$ and hence, $\delta(P_\ell^{j-1})\subseteq \delta(P_\ell^{j-1}\cup C_j)$. Consequently,  $\delta(P_\ell^{j-1}\cup C_j)=\delta(P_\ell^{j-1})$.

%Therefore, $C_j$ is merged with $V_{i'}^{j-1}$ for some $i'\in[k]$, resulting in $V_{i'}^j=V_{i'}^{j-1}\cup C_j$ and $V_i^j=V_i^{j-1}$ for all $i\neq i'$. This also implies $C_1\cup\ldots\cup C_{j}\subseteq\left(\cup_{i=1}^kV_i^{j-1}\right)\cup C_j=\cup_{i=1}^kV_i^{j}$, completing our induction step.

%By induction, we have $C_1\cup\ldots\cup C_t\subseteq \cup_{i=1}^k V_i^t$. Moreover, we have $U_i\subseteq V_i^t$ for all $i\in[k]$ by initialization. Hence, $\cup_{i=1}^k V_i=\cup_{i=1}^k V_i^t=V$.

%it returns the requested partition only when it exists. We now show that if such a partition exists, then This completes the proof for correctness.

We now bound the run-time. We can verify if there exists $i\in [k]$ such that $\delta(P_i\cup C_j)=\delta(P_i)$ in time $O(mk)$ \wnote{can we verify hyperedge intersection in constant time, or do we need a tilde here?}. The number of iterations of the for-loop is $t\le n$. Hence, the total run-time is $O(nmk)$. 
%the total number of inner for-loops is $O(nk)$ because $t\leq k$. Each inner for-loop can be implemented in $O(m)$ time, resulting in a total run time of $O(nmk)$.
%\knote{Check the run-time}
\end{proof}

Next, we address the problem of enumerating all \minmaxkcutsets. For this, we define a sub-problem---namely \enumkcutsetreps. The input here is a hypergraph $G=(V,E)$ and a fixed positive integer $k$ (e.g., $k=2, 3, 4, \ldots$). The goal is to 
enumerate a family $\family$ of $k$-cut-set representatives satisfying the following two properties: 
%of all optimum $k$-partitions for \mmh---i.e., 
\begin{enumerate}[(1)]
    \item every $k$-tuple $(U_1, \ldots, U_k)$ in the family $\family$ will be the $k$-cut-set representative of some optimum $k$-partition $(V_1, \ldots, V_k)$ for \mmh and 
    \item for every optimum $k$-partition $(V_1, \ldots, V_k)$ for \mmh, the family $\family$ contains a $k$-cut-set representative $(U_1, \ldots, U_k)$ of $(V_1, \ldots, V_k)$. 
\end{enumerate}
We note that if the solution to \enumkcutsetreps is a family $\family$, then returning $\{\cup_{i=1}^k \delta(U_i): (U_1, \ldots, U_k)\in \family \}$ solves \enumMMh. Hence, it suffices to solve \enumkcutsetreps in order to prove Theorem \ref{thm:minmax-enumeration}. We now design an algorithm for \enumkcutsetreps. 
%Theorem \ref{thm:minmax-enumeration} follows from Theorem \ref{Thm: hyp minmax-2}. 
%be used to solve \enumMMh by returning 


\iffalse
%Essentially, we design an algorithm to find a family of representatives for all \minmax $k$-partitions. 
We note that enumerating the family $\family$ of $k$-cut-set representatives of all optimum $k$-partitions for \mmh suffices to enumerate all \minmaxkcutsets: for this, it suffices to consider the family $\{\cup_{i=1}^k \delta(U_i): (U_1, \ldots, U_k)\in \family \}$. 
%Moreover, knowing a $k$-cut-set representative $(U_1, \ldots, U_k)$ of a $k$-partition $(V_1, V_2, \ldots, V_k)$ allows one to recover the $k$-cut-set $F=\delta(V_1, \ldots, V_k)$ since $F=\cup_{i=1}^k \delta(U_i)$. 
%Thus, in order to enumerate all \minmaxkcutsets, it suffices to enumerate $k$-cut-set representatives for \emph{all} optimum $k$-partitions for \mmh. 
We now design an algorithm that returns the family of $k$-cut-set representatives of all optimum $k$-partitions for \mmh---see Theorem \ref{Thm: hyp minmax-2}. Theorem \ref{thm:minmax-enumeration} follows from Theorem \ref{Thm: hyp minmax-2}. 
\fi


\begin{theorem}\label{Thm: hyp minmax-2}
Let $G=(V,E)$ be a $n$-vertex hypergraph of size $p$ with $m$ hyperedges and let $k$ be an integer. Then, Algorithm Enum-MinMax$(G, k)$ in Figure \ref{Algo: hyp minmax-2} 
%returns the family of 
%cutsets of all \minmax $k$-partitions in $G$ and 
%$k$-cut-set representatives of all optimum $k$-partitions for \mmh and 
solves \enumkcutsetreps 
and  
it can be implemented to run in time $O(n^{4k^2-2k+1}mp)$. Moreover, the cardinality of the family returned by the algorithm is $O(n^{4k^2-2k})$.
\end{theorem}

%\wnote{Algorithm names in theorem and figure don't match}
\begin{figure*}[ht]
\centering\small
\begin{algorithm}
\textul{Algorithm Enum-MinMax$(G=(V,E),k)$}\+
\\{\bf Input:} Hypergraph $G=(V,E)$ and an integer $k\geq 2$
\\{\bf Output:} Family $\mathcal{F}$ of $k$-cut-set representatives of all optimum $k$-partitions\+\+
\\$\,\;$for \mmh\-\- 
\\Initialize $\mathcal{C}\gets\emptyset$, $\mathcal{D}\gets\emptyset$, and  $\mathcal{F}\gets\emptyset$
\\For each pair $(S,T)$ such that $S,T\subseteq V$ with $S\cap T=\emptyset$ and $|S|$, $|T|\leq 2k-1$ \+
\\ Compute the source minimal minimum $(S,T)$-terminal cut $(U,\complement{U})$
\\$\mathcal{C}\gets\mathcal{C}\cup\{U\}$\-
\\For all $(U_1,\ldots, U_k)\in\mathcal{C}^k$ such that $U_1,\ldots, U_k$ are pairwise disjoint\+
\\If Recover-Partition$(G,U_1,\ldots, U_k)$ returns a $k$-partition\+ %$(P_1,\ldots,P_k)$\+
\\$\mathcal{D}\gets\mathcal{D}\cup\{(U_1,\ldots,U_k)\}$\-\-
\\$\lambda \leftarrow \min\{\max_{i\in [k]}d(U_i): (U_1, \ldots, U_k)\in \mathcal{D}\} $
\\For all $(U_1, \ldots, U_k)\in \mathcal{D}$ such that $\max_{i\in [k]}d(U_i)=\lambda$:\+
\\$\mathcal{F}\leftarrow \mathcal{F}\cup\{(U_1, \ldots, U_k)\}$\-
\\ Return $\mathcal{F}$
%\\Among all $k$-cut-sets $\{\cup_{i=1}^k\delta(U_i):(U_1,\ldots,U_k)\in\mathcal{D}\}$, return the subfamily of cheapest ones
%\\Return $\mathcal{F}\gets\{\cup_{i=1}^k\delta(U_i):(U_1,\ldots,U_k)\in\mathcal{D},\max_{i\in[k]}d(U_i)=\min_{(U_1',\ldots,U_k')\in\mathcal{D}}\max_{i\in[k]}d(U_i')\}$
\end{algorithm}
\caption{Algorithm in Theorem \ref{Thm: hyp minmax-2}}
\label{Algo: hyp minmax-2}
\end{figure*}
%\knote{Need to be clear about ``cheapest ones''.}

\begin{proof}
%We will show that Algorithm \ref{Algo: hyp minmax-2} works as described in Theorem \ref{Thm: hyp minmax-2}. 

We begin by showing correctness---i.e., the family $\family$ returned by the algorithm satisfies properties (1) and (2) mentioned in the definition of \enumkcutsetreps. 
By the second for-loop, each $k$-tuple added to the collection $\mathcal{D}$ is a $k$-cut-set representative of some $k$-partition (it need not necessarily be a $k$-cut-set representative of an optimum  $k$-partition for \mmh). The algorithm returns a subfamily of $\mathcal{D}$ and hence, it returns a subfamily of $k$-cut-set representatives. 
We only have to show that a $k$-cut-set representative of an arbitrary optimum $k$-partition for \mmh is present in the family $\mathcal{D}$; this will guarantee that the subfamily $\family$ returned by the algorithm indeed satisfies properties (2) as well as (1) (property (1) will be satisfied owing to the construction of the family $\family$ from the family $\mathcal{D}$). 
%consists of cut-set representatives of all optimum $k$-partitions for \mmh. 

%The last step of the algorithm considers only $k$-cut-sets, so the algorithm returns a subfamily of $k$-cut-sets. We only have to show that every \minmax $k$-cut-set is in the family $\mathcal{F}$; this will also guarantee that every $k$-cut-set in the returned subfamily is indeed a \minmax $k$-cut-set.

Let $\optmm$ denote the optimum value of a \minmax $k$-partition in $G$ and let $\optk$ denote the optimum value of a minimum $k$-cut in $G$. We note that $\optmm\le \optk$. This is because, if $(P_1, \ldots, P_k)$ is a $k$-partition with minimum $|\delta(P_1, \ldots, P_k)|$ (i.e., an optimum $k$-partition for \hkcut), then 
\[
\optmm\le \max_{i\in [k]}|\delta(P_i)|\le |\delta(P_1, \ldots, P_k)|=\optk. 
\]

Let $(V_1, \ldots, V_k)$ be an arbitrary \minmax $k$-partition. We will show that the family $\mathcal{F}$ returned by the algorithm contains a $k$-cut-set representative of $(V_1, \ldots, V_k)$. 
%Let $(V_1, \ldots, V_k)$ be a \minmax $k$-partition. 
%Let us fix a \minmax $k$-partition $(V_1,\ldots,V_k)$. 
We have that $d(V_i)\leq \optmm\le \optk$ for all $i\in [k]$. Hence, by Theorems \ref{theorem: structure thm 1} and \ref{thm:cut-set-recovery}, there exist subsets $S_i\subseteq V_i$, $T_i\subseteq V-V_i$ with $|S_i|,|T_i|\leq 2k-1$ such that the source minimal minimum $(S_i,T_i)$-terminal cut $(U_i,\complement{U_i})$ satisfies $\delta(U_i)=\delta(V_i)$ for all $i\in [k]$. 
%and consequently $U_i\in \mathcal{C}$. 
Source minimality of the cut $(U_i,\complement{U_i})$ also guarantees that $U_i\subseteq V_i$ for all $i\in[k]$. Hence, the $k$-tuple $(U_1, \ldots, U_k)$ is a $k$-cut-set representative of $(V_1, \ldots, V_k)$. It remains to show that this $k$-tuple is indeed present in the families $\mathcal{D}$ and $\mathcal{F}$. 
We note that the sets $U_1, \ldots, U_k$ are added to $\mathcal{C}$ in the first for-loop. Since the $k$-tuple $(U_1, \ldots, U_k)$ is a $k$-cut-set representative of the $k$-partition $(V_1, \ldots, V_k)$, the $k$-tuple $(U_1, \ldots, U_k)$ will be added to $\mathcal{D}$ in the second for-loop. Since $\mathcal{D}$ contains only $k$-cut-set representatives of $k$-partitions, it follows that $\lambda = \optmm$ and $(U_1, \ldots, U_k)$ will be added to $\mathcal{F}$ in the third for-loop. Hence, the $k$-cut-set representative $(U_1, \ldots, U_k)$ of the optimum $k$-partition $(V_1, \ldots, V_k)$ of \mmh is present in the family $\mathcal{F}$ returned by the algorithm. 

\iffalse
The second for-loop will add the tuple $(U_1, \ldots, U_k)$ 
are present in $\mathcal{C}$ and they are pairwise disjoint. 
%Hence, the set $U_i$ is in the collection $\mathcal{C}$. 
%By construction of Algorithm \ref{Algo: hyp minmax-2}, disjoint subsets $U_1,\ldots, U_k$ are all in $\mathcal{C}$. 
By existence of $(V_1,\ldots,V_k)$, the $k$-tuple $(U_1,\ldots,U_k)$ is added to $\mathcal{D}$.

For every $(U'_1,\ldots,U'_k)\in\mathcal{D}$, there exists a $k$-partition $(V'_1,\ldots,V'_k)$ such that $U'_i\subseteq V'_i$ and $\delta(U'_i\delta(V'_i)$ for all $i\in[k]$. Thus, we have
\[\max_{i\in[k]}d(U'_i)\geq\optmm=\max_{i\in[k]}d(U_i),\]
and hence $\cup_{i=1}^k\delta(U_i)\in\mathcal{F}$.
\fi

The bound on the size of the family $\mathcal{F}$ returned by the algorithm is
\[
|\mathcal{F}|\le |\mathcal{D}| \le |\mathcal{C}|^k = O(n^{k(4k-2)}). 
\]
%The size of $\mathcal{F}$ is bounded by the size of $\mathcal{D}$, which is further bounded by the size of $\mathcal{C}^k$. The size of $\mathcal{C}$ is $O(n^{4k-2})$. Therefore, we have $|\mathcal{F}|\leq n^{4k^2-2k}$.

Next, we bound the run time of the algorithm. 
The first for-loop can be implemented to run in time $O(n^{4k-2})T(n, p)$. 
The second for-loop executes the algorithm from Theorem \ref{Thm: hyp minmax-1}  $O(n^{4k^2-2k})$ times and hence, the second for-loop can be implemented to run in time $O(n^{4k^2-2k+1}mp)$. The computation of $\lambda$ and the third for-loop can be implemented to run in time $O(|\mathcal{D}|)=O(n^{4k^2-2k})$. 
%The last step can be implemented to run in time at most $O(|\mathcal{D}|)\le n^{4k^2-2k}$. 
Hence, the total run-time is $O(n^{4k-2})T(n,p)+O(n^{4k^2-2k+1}mp)$. We recall that $T(n, p)=O(n p)$ and hence, the total run-time is $O(n^{4k^2-2k+1}mp)$.

%The run time is dominated by the second for-loop, which runs Algorithm \ref{Algo: hyp minmax-1} $n^{4k^2-2k}$ times. This results in a total run time of $O(n^{4k^2-2k+1}mp)$.


\end{proof}

\knote{Consider the spanning-hyperedge-example. Number of optimum $2$-partitions is $2^n$. Number of minimum cut-sets is $1$. Is it immediately clear that there exists a family $\family$ of cut-set representatives satisfying (1) and (2) such that $|\family|=poly(n)$? We should give a simple argument for this and highlight it in the technical overview section.}



